Toward Human Understanding with Controllable Synthesis

Training methods to perform robust 3D human pose and shape (HPS) estimation requires diverse training images with accurate ground truth. While BEDLAM demonstrates the potential of traditional procedural graphics to generate such data, the training images are clearly synthetic. In contrast, generative image models produce highly realistic images but without ground truth. Putting these methods together seems straightforward: use a generative model with the body ground truth as controlling signal. However, we find that, the more realistic the generated images, the more they deviate from the ground truth, making them inappropriate for training and evaluation. Enhancements of realistic details, such as clothing and facial expressions, can lead to subtle yet significant deviations from the ground truth, potentially misleading training models. We empirically verify that this misalignment causes the accuracy of HPS networks to decline when trained with generated images. To address this, we design a controllable synthesis method that effectively balances image realism with precise ground truth. We use this to create the Generative BEDLAM (Gen-B) dataset, which improves the realism of the existing synthetic BEDLAM dataset while preserving ground truth accuracy. We perform extensive experiments, with various noise-conditioning strategies, to evaluate the tradeoff between visual realism and HPS accuracy. We show, for the first time, that generative image models can be controlled by traditional graphics methods to produce training data that increases the accuracy of HPS methods.

==> graphs/fid_vs_noise.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}[t]{0.48\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \begin{axis}[
%                 xlabel={Noise Level},
%                 ylabel={FID Score},
%                 legend style={at={(0.5,-0.3)}, anchor=north, legend columns=3},
%                 ymajorgrids=true,
%                 grid style=dashed,
%                 xmin=0.2, xmax=1.0,
%                 ymin=130, ymax=170,
%                 xtick={0.3, 0.5, 0.7, 0.9},
%                 width=\textwidth,
%                 height=0.6\textwidth
%             ]
%             \addplot[
%                 color=blue,
%                 mark=square*,
%                 ]
%                 coordinates {
%                 (0.3,146.25)(0.5,144.56)(0.7,152.04)(0.9,161.58)
%                 };
%                 \addlegendentry{3DPW}
                
%             \addplot[
%                 color=red,
%                 mark=*,
%                 ]
%                 coordinates {
%                 (0.3,139.90)(0.5,140.50)(0.7,145.99)(0.9,152.75)
%                 };
%                 \addlegendentry{EMDB}
                
%             \addplot[
%                 color=green,
%                 mark=triangle*,
%                 ]
%                 coordinates {
%                 (0.3,144.59)(0.5,141.17)(0.7,145.03)(0.9,149.27)
%                 };
%                 \addlegendentry{RICH}
                
%             \end{axis}
%         \end{tikzpicture}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.48\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \begin{axis}[
%                 xlabel={Noise Level},
%                 ylabel={Second Metric Score},
%                 legend style={at={(0.5,-0.3)}, anchor=north, legend columns=3},
%                 ymajorgrids=true,
%                 grid style=dashed,
%                 xmin=0.2, xmax=1.0,
%                 ymin=90, ymax=160,
%                 xtick={0.3, 0.5, 0.7, 0.9},
%                 width=\textwidth,
%                 height=0.6\textwidth
%             ]
%             \addplot[
%                 color=blue,
%                 mark=square*,
%                 ]
%                 coordinates {
%                 % (0.3,97.56)(0.5,98.37)(0.7,101.29)(0.9,104.38)
%                 (0.3,97.90)(0.5,98.37)(0.7,101.29)(0.9,104.38)
%                 % (0.3,113.63)(0.5,115.35)(0.7,118.37)(0.9,121.50)
%                 % (0.3,114.03)(0.5,115.35)(0.7,118.37)(0.9,121.50)
%                 };
%                 \addlegendentry{3DPW}
                
%             \addplot[
%                 color=red,
%                 mark=*,
%                 ]
%                 coordinates {
%                 % (0.3,147.71)(0.5,142.42)(0.7,145.12)(0.9,146.30)
%                 (0.3,140.42)(0.5,142.42)(0.7,145.12)(0.9,146.30)
%                 % (0.3,171.41)(0.5,165.41)(0.7,167.83)(0.9,171.56)
%                 % (0.3,163.06)(0.5,165.41)(0.7,167.83)(0.9,171.56)
%                 };
%                 \addlegendentry{EMDB}
                
%             \addplot[
%                 color=green,
%                 mark=triangle*,
%                 ]
%                 coordinates {
%                 % (0.3,122.14)(0.5,118.08)(0.7,117.22)(0.9,122.82)
%                 (0.3,117.01)(0.5,118.08)(0.7,117.22)(0.9,122.82)
%                 % (0.3,134.04)(0.5,132.29)(0.7,130.93)(0.9,137.31)
%                 % (0.3,130.28)(0.5,132.29)(0.7,130.93)(0.9,137.31)
%                 };
%                 \addlegendentry{RICH}
                
%             \end{axis}
%         \end{tikzpicture}
%     \end{minipage}
%     \caption{Comparison of FID Score and Second Metric Score vs Noise Level for different datasets}
%     \label{fig:comparison_metrics}
% \end{figure*}


% \begin{figure}[t]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             width=\columnwidth, % Adjust the width to fit within a column
%             % height=0.3\columnwidth, % Adjust the height proportionally
%             xlabel={Noise level},
%             ylabel={FID score},
%             xtick={0.3,0.5,0.7,0.9},
%             xticklabels={0.3,0.5,0.7,0.9},
%             ytick={140, 145, 150, 155, 160, 165},
%             bar width=0.45cm,
%             ylabel near ticks,
%             xlabel near ticks,
%             legend style={at={(1,1.05)}, anchor=south east},
%             grid=major,
%             enlarge x limits=0.15,
%             enlarge y limits=0.15,
%             cycle list name=color list,
%             nodes near coords,
%             every node near coord/.append style={font=\footnotesize}
%         ]
%         % Define bar colors manually
%         \addplot[
%             ybar,
%             fill=blue,
%             mark=none
%         ]
%         coordinates {(0.3, 146.25)};
        
%         \addplot[
%             ybar,
%             fill=red,
%             mark=none
%         ]
%         coordinates {(0.5, 144.56)};
        
%         \addplot[
%             ybar,
%             fill=green,
%             mark=none
%         ]
%         coordinates {(0.7, 152.04)};
        
%         \addplot[
%             ybar,
%             fill=orange,
%             mark=none
%         ]
%         coordinates {(0.9, 161.58)};
%         coordinates {
%             (0.3, 146.25) (0.5, 144.56) (0.7, 152.04) (0.9, 161.58)
%         };
%         \end{axis}
%     \end{tikzpicture}
%     \caption{Bar plot of given values with different colors for each bar.}
%     \label{fig:barplot}
% \end{figure}

\begin{figure*}[h]
    \centering
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Noise Level},
                ylabel={MPJPE (mm)},
                legend style={at={(0.5,-0.3)}, anchor=north, legend columns=3},
                ymajorgrids=true,
                grid style=dashed,
                xmin=0.2, xmax=1.0,
                ymin=90, ymax=160,
                xtick={0.3, 0.5, 0.7, 0.9},
                width=\textwidth,
                height=0.6\textwidth
            ]
            \addplot[
                color=blue,
                mark=square*,
                ]
                coordinates {
                % (0.3,97.56)(0.5,98.37)(0.7,101.29)(0.9,104.38)
                (0.3,97.90)(0.5,98.37)(0.7,101.29)(0.9,104.38)
                % (0.3,113.63)(0.5,115.35)(0.7,118.37)(0.9,121.50)
                % (0.3,114.03)(0.5,115.35)(0.7,118.37)(0.9,121.50)
                };
                \addlegendentry{3DPW}
                
            \addplot[
                color=red,
                mark=*,
                ]
                coordinates {
                % (0.3,147.71)(0.5,142.42)(0.7,145.12)(0.9,146.30)
                (0.3,140.42)(0.5,142.42)(0.7,145.12)(0.9,146.30)
                % (0.3,171.41)(0.5,165.41)(0.7,167.83)(0.9,171.56)
                % (0.3,163.06)(0.5,165.41)(0.7,167.83)(0.9,171.56)
                };
                \addlegendentry{EMDB}
                
            \addplot[
                color=green,
                mark=triangle*,
                ]
                coordinates {
                % (0.3,122.14)(0.5,118.08)(0.7,117.22)(0.9,122.82)
                (0.3,117.01)(0.5,118.08)(0.7,117.22)(0.9,122.82)
                % (0.3,134.04)(0.5,132.29)(0.7,130.93)(0.9,137.31)
                % (0.3,130.28)(0.5,132.29)(0.7,130.93)(0.9,137.31)
                };
                \addlegendentry{RICH}
                
            \end{axis}
        \end{tikzpicture}
    \caption{Bar plot of given values with different colors for each bar.}
    \label{fig:barplot}
\end{figure*}

==> img/captions/realism_vs_faith.tex <==
\begin{figure}
\begin{center}
   \includegraphics[width=\linewidth]{author-kit-3DV2025-v1/img/noise_variation.pdf}
\end{center}
   \caption{\textbf{Faithfulness vs Realism}. It shows how the generated image becomes more realistic as more noise is added but it starts diverging from the original image.}
\label{fig:faith_realism}
\end{figure}

==> sec/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

\hf{the intro story would need a turn from selling our hybrid solution as novel and useful to selling this solution as natural decision but surprising not working as expected, then leads to the intriguing discussion of alignment gap of controllable synthesis and it is a pressing matter for using controllable synthesis for visual understanding tasks like HPS}
Training neural networks to accurately estimate 3D human pose and shape (HPS) requires large amounts of training data.
Ideally, this data includes paired images with ground truth pose and shape parameters, e.g.~parameters of a parametric body model like SMPL \cite{loper2015smpl}.
Capturing real images with ground truth data is hard so many methods rely on pseudo ground truth estimated from 2D data.
This can introduce errors and bias.
An alternative is synthetic data but, until recently, the domain gap between real and synthetic images meant that such data was insufficient to train networks without also using real data.
The BEDLAM dataset \cite{black2023bedlam} shows that traditional graphics methods can produce images with ground truth data of sufficient complexity and realism that training only on the synthetic data produces state of the art (SOTA) accuracy.
Despite this, images in the BEDLAM dataset are still very obviously synthetic.
Thus, there remains a domain gap between synthetic training images and real test images. \hf{to push the realism axis}

\hf{Recent work on deep generative models have shown promising results for generating fully realistic images of synthetic humans with an effectively infinite variation in clothing, hair, lighting, skin tone, etc. Together with controllable synthesis methods like ControlNet \cite{zhang2023adding}, it provides a solution by conditioning the generated image on properties like the 2D pose of the person.} 
% These images, however, cannot be use as training data because they lack ground truth 3D pose and shape information.
Here we ask whether the accuracy of 3D HPS can be improved by more realistic imagery \hf{enhanced by generative models}?
% Methods like ControlNet \cite{zhang2023adding} could provide a solution by conditioning the generated image on properties like the 2D pose of the person.
While results look good they still lack 3D pose information and, importantly, 3D body shape information.
\hf{alignment gap between the ground truth control signal and its generation}

\hf{the hybrid solution is proposed to minimize the alignment gap}
Here we address this problem by combining the best of traditional and generative methods.
Specifically, we take the BEDLAM dataset and ``upgrade" the visual appearance using generative models.
We find that doing this, while preserving the key properties of the ground truth, is non-trivial.
We present a pipeline that changes things like clothing, without impacting the body shape.
We increase the realism of the faces and add hair and shoes, which are missing or often missing in BEDLAM.
The result is a new dataset of images in which the people are much closer to photorealistic but the ground truth body shape and pose is unchanged.
See Fig.~\ref{fig:teaser} for comparisons between BEDLAM and our new Generative BEDLAM (or GenB) dataset.

The key question is whether this increase in visual realism translates into improved metric accuracy.
Given the large amount of augmentations applied to training images, this is not a prior obvious.
In a sense, we want to train network results to be invariant to variations in image appearance so making images more realistic may just mean that the network ignores this.
In fact, we find that GenB results in a significant performance gain, resulting in a new state of the art.


To evaluate this, we perform an extensive evaluation....
We train HMR \cite{hmr} with the original BEDLAM dataset and GenB.
We find that training on GenB improves accuracy on real test datasets, 3DPW, RICH, HMDB, by XX, XX, and XX percent respectively.
HMR is based on a convolutional architecture and the most accurate recent methods are based on transformers (\cite{neuripssynbodypaper,4dhumans}.
We take the 4DHumans architecture and train it using only synthetic data (both BEDLAM and GenB).
We find that using only BEDLAM or GenB training data, 4DHumans is XX and and XX percent more accurate than the original method, which is trained are XX real images.
Again we find a XX percent improvement using GenB over BEDLAM.
Finally, we combine the bounding box idea from CLIFF with the 4DHumans architecture and train on GenB.
This results in the most accurate method and the current SOTA.

In summary, we 
(1) provide a process to upgrade synthetic data like BEDLAM using generative models while preserving the ground truth body shape and pose;
(2) provide a new dataset, GenB, that can be used to train HPS regressors to achieve SOTA accuracy;
(3) extensively evaluate existing methods trained on GenB,
(4) combine ideas from the best convolutional and transformer-based methods to achieve a new level of accuracy.
The dataset, code to generate the dataset, trained models, and model training code will be available for research purposes.

